The use of Generative Adversarial Networks to characterise new physics in multi-lepton final states at the LHC

Semi-supervision in Machine Learning can be used in searches for new physics where the signal plus background regions are not labelled. This strongly reduces model dependency in the search for signals Beyond the Standard Model. This approach displays the drawback in that over-fitting can give rise to fake signals. Tossing toy Monte Carlo (MC) events can be used to estimate the corresponding trials factor through a frequentist inference. However, MC events that are based on full detector simulations are resource intensive. Generative Adversarial Networks (GANs) can be used to mimic MC generators. GANs are powerful generative models, but often suffer from training instability. We henceforth show a review of GANs. We advocate the use of Wasserstein GAN (WGAN) with weight clipping and WGAN with gradient penalty (WGAN-GP) where the norm of gradient of the critic is penalized with respect to its input. Following the emergence of multi-lepton anomalies, we apply GANs for the generation of di-leptons final states in association with $b$-quarks at the LHC. A good agreement between the MC and the WGAN-GP generated events is found for the observables selected in the study.

==> main_res.tex <==
\begin{figure}[H]
    \begin{center}
% \fbox{}
    \includegraphics[height=8cm, width=15cm]{plots_loc/Image_4_3a.jpg}
    \end{center}
\caption{Results on the best performing epoch of the WGAN-GP, with WGAN-GP generated event (in orange) and original MC (in blue) and their associated mean values.}
\label{fig:architecture_scope}
\end{figure}

==> tables_loc/table_fig.tex <==
\begin{figure}[H]
    \begin{center}
    \includegraphics[width=\textwidth,clip]{table_fig.png}
    \end{center}
\caption{Tabulated mean values of MC, WGAN-GP events and their relative mean difference.}
\label{fig:table}
\end{figure}

